ActFusion: a Unified Diffusion Model for Action Segmentation and Anticipation

Temporal action segmentation and long-term action anticipation are two popular vision tasks for the temporal analysis of actions in videos. Despite apparent relevance and potential complementarity, these two problems have been investigated as separate and distinct tasks. In this work, we tackle these two problems, action segmentation and action anticipation, jointly using a unified diffusion model dubbed ActFusion. The key idea to unification is to train the model to effectively handle both visible and invisible parts of the sequence in an integrated manner; the visible part is for temporal segmentation, and the invisible part is for future anticipation. To this end, we introduce a new anticipative masking strategy during training in which a late part of the video frames is masked as invisible, and learnable tokens replace these frames to learn to predict the invisible future. Experimental results demonstrate the bi-directional benefits between action segmentation and anticipation. ActFusion achieves the state-of-the-art performance across the standard benchmarks of 50 Salads, Breakfast, and GTEA, outperforming task-specific models in both of the two tasks with a single unified model through joint learning.

==> sections_sup/10_fullresults.tex <==
\section{Full results}
\label{sec_sup:full_results}
Table~\ref{tab:masking} presents the full results of Table 4, which were omitted due to the lack of space.
\input{tables/table_masking}

==> sections_sup/3_training_objective.tex <==
\section{Training objective}
\label{sec_sup:training_obj}
In this section, we provide a detailed formulation of the training objective outlined in Sec.~4.4. 
The training objective consists of a summation of the encoder loss and the decoder loss.

\textbf{Training losses.}
Three types of losses are utilized during training both the encoder and the decoder, which are the cross-entropy loss $\mathcal{L}_\mathrm{ce}$, the boundary smoothing loss $\mathcal{L}_\mathrm{smo}$~\cite{farha2019ms}, and the boundary alignment loss $\mathcal{L}_\mathrm{bd}$~\cite{liu2023diffusion}.

Given the ground-truth action label $\bm{A}^0\in\mathbb{R}^{T \times K}$ and the predictions $\hat{\bm{A}}\in\mathbb{R}^{T \times K}$, the cross entropy loss is defined by:
\begin{align}
    \mathcal{L}_\mathrm{ce}(\bm{A}^0, \bm{\hat{A}}) &= -\sum^{T}_{i=1}\sum^{K}_{j=1} \bm{A}^{0}_{i,j}\log\hat{\bm{A}}_{i,j}.
\end{align}
To prevent over-segmentation errors, a temporal smooth loss between adjacent frames based on a truncated mean squared error over the frame-wise log probabilities~\cite{farha2019ms} are defined by:
\begin{align}
    \mathcal{L}_\mathrm{smo}(\bm{\hat{A}}) &= \frac{1}{(T-1)K}\sum_{i=1}^{T-1}\sum_{j=1}^{K}(\log\bm{\hat{A}}_{i,j}-\log\bm{\hat{A}}_{i+1,j})^2,
\end{align}
where the difference of the log probabilities of two adjacent frames is truncated with a threshold value.
For precise boundary detection, the boundary alignment loss~\cite{liu2023diffusion} is employed based on the binary cross-entropy loss:
\begin{equation}
    \begin{split}
        \mathcal{L}_\mathrm{bd}(\bm{\hat{A}}) = \frac{1}{T-1}\sum_{i=1}^{T-1}&\{-\bm{B}_i\log(1-\bm{\hat{A}}_i \cdot \bm{\hat{A}}_{i+1}) \\ &-(1-\bm{B}_i)\log(\bm{\hat{A}}_i \cdot \bm{\hat{A}}_{i+1})\},
    \end{split}
\end{equation}
where $\bm{B}$ represents a softened version of the ground-truth action boundary, achieved through a Gaussian kernel.

\textbf{Encoder losses.}
Given the ground-truth action sequences $\bm{A}^0$ and the encoder predictions $\hat{\bm{A}}^\mathrm{enc}$, the overall encoder losses are defined by:
\begin{align}
    \mathcal{L}^\mathrm{enc} &= \lambda^\mathrm{enc}_\mathrm{ce}\mathcal{L}^\mathrm{enc}_\mathrm{ce} + \lambda^\mathrm{enc}_\mathrm{smo}\mathcal{L}^\mathrm{enc}_\mathrm{smo} +
    \lambda^\mathrm{enc}_\mathrm{bd}\mathcal{L}^\mathrm{enc}_\mathrm{bd},\\
    \mathcal{L}^\mathrm{enc}_\mathrm{ce} &= \mathcal{L}_\mathrm{ce}(\bm{A}^0, \bm{\hat{A}}^\mathrm{enc}),\\
    \mathcal{L}^\mathrm{enc}_\mathrm{smo} &= \mathcal{L}_\mathrm{smo}(\bm{\hat{A}}^\mathrm{enc}), \\
    \mathcal{L}^\mathrm{enc}_\mathrm{bd} &= \mathcal{L}_\mathrm{bd}(\bm{\hat{A}}^\mathrm{enc}),
\end{align}
where $\lambda^\mathrm{enc}$ denotes a scaling factor.

\textbf{Decoder losses.}
Given the ground-truth action sequences $\bm{A}^0$ and the decoder predictions $\hat{\bm{A}}^0$, the overall decoder losses are defined by:
\begin{align}
    \mathcal{L}^\mathrm{dec} &= \lambda^\mathrm{dec}_\mathrm{ce}\mathcal{L}^\mathrm{dec}_\mathrm{ce} + \lambda^\mathrm{dec}_\mathrm{smo}\mathcal{L}^\mathrm{dec}_\mathrm{smo} +
    \lambda^\mathrm{dec}_\mathrm{bd}\mathcal{L}^\mathrm{dec}_\mathrm{bd},\\
    \mathcal{L}^\mathrm{dec}_\mathrm{ce} &= \mathcal{L}_\mathrm{ce}(\bm{A}^0, \bm{\hat{A}}^0),\\
    \mathcal{L}^\mathrm{dec}_\mathrm{smo} &= \mathcal{L}_\mathrm{smo}(\bm{\hat{A}}^0), \\
    \mathcal{L}^\mathrm{dec}_\mathrm{bd} &= \mathcal{L}_\mathrm{bd}(\bm{\hat{A}}^0),
\end{align}
where $\lambda^\mathrm{dec}$ denotes a scaling factor.

\textbf{Final losses.}
The overall training loss $\mathcal{L}^\mathrm{total}$ is a summation of the encoder and decoder losses, defined as:
\begin{align}
    \mathcal{L}^\mathrm{total} = \mathcal{L}^\mathrm{enc} + \mathcal{L}^\mathrm{dec}.
\end{align}
